Multi-speaker Text-to-speech Training with Speaker Anonymized Data

The trend of scaling up speech generation models poses a threat of biometric information leakage of the identities of the voices in the training data, raising privacy and security concerns. In this paper, we investigate training multi-speaker text-to-speech (TTS) models using data that underwent speaker anonymization (SA), a process that tends to hide the speaker identity of the input speech while maintaining other attributes. Two signal processing-based and three deep neural network-based SA methods were used to anonymize VCTK, a multi-speaker TTS dataset, which is further used to train an end-to-end TTS model, VITS, to perform unseen speaker TTS during the testing phase. We conducted extensive objective and subjective experiments to evaluate the anonymized training data, as well as the performance of the downstream TTS model trained using those data. Importantly, we found that UTMOS, a data-driven subjective rating predictor model, and GVD, a metric that measures the gain of voice distinctiveness, are good indicators of the downstream TTS performance. We summarize insights in the hope of helping future researchers determine the goodness of the SA system for multi-speaker TTS training.

==> correlations-sim-percentage.tex <==
\begin{table}[t]
\centering
\caption{Linear correlation coefficients between the SA evaluation metrics and the TTS evaluation results. Bold indicates a strong correlation ($>0.7$).}
\label{tab:correlation-sim-percentage}
\begin{tabular}{@{}ccc|cc@{}}
\toprule
                                                                         &                       &        & \multicolumn{2}{c}{TTS evaluation} \\ \cmidrule(l){4-5} 
                                                                         &                       &        & TTS-NAT          & TTS-SIM         \\ \midrule
\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}SA\\ evaluation\end{tabular}} & \multirow{4}{*}{Obj.} & WER    & \textbf{-0.785}  & -0.559          \\
                                                                         &                       & EER    & 0.231            & -0.035          \\
                                                                         &                       & GVD    & -0.220           & \textbf{0.773}  \\
                                                                         &                       & UTMOS  & \textbf{0.874}   & 0.372           \\ \cmidrule(l){2-5} 
                                                                         & \multirow{2}{*}{Sub.} & SA-NAT & \textbf{0.929}   & 0.498           \\
                                                                         &                       & SA-SIM & 0.477            & \textbf{0.892}  \\ \bottomrule
\end{tabular}
\vspace{-10pt}
\end{table}
